GFET Lab: A Graphene Field-Effect Transistor TCAD Tool

Graphene field-effect transistors (GFETs) are experimental devices which are increasingly seeing commercial and research applications. Simulation and modelling forms an important stage in facilitating this transition, however the majority of GFET modelling relies on user implementation. To this end, we present GFET Lab, a user-friendly, open-source software tool for simulating GFETs. We first provide an overview of approaches to device modelling and a brief survey of GFET compact models and limitations. From this survey, we identify three key criteria for a suitable predictive model for circuit design: it must be a compact model; it must be SPICE-compatible; it must have a minimal number of fitting parameters. We selected Jimenez's drain-current model as it best matched these criteria, and we introduce some modifications to improve the predictive properties, namely accounting for saturation velocity and the asymmetry in n- and p-type carrier mobilities. We then validate the model by comparing GFETs simulated in our tool against experimentally-obtained GFET characteristics with the same materials and geometries and find good agreement between GFET Lab and experiment. We demonstrate the ability to export SPICE models for use in higher level circuit simulations and compare SPICE simulations of GFETs against GFETs simulated in GFET Lab, again showing good agreement. Lastly, we provide a brief tutorial of GFET Lab to demonstrate and encourage its use as a community-developed piece of software with both research and educational applications.

==> methodology.tex <==
%
%	Keep the lines in the LaTeX file short (see below).
%	This makes it easier to read and also makes checking
%	diffs easier since most Unix diff tools are line-based:
%	If a whole paragraph is a single line, then `diff` will
%	flag it up as changed even if you just changed a comma or
%	spacing in one sentence.
%
\section{Methodology}
\label{section:methodology}
The methodology section should state clearly what steps you followed,
in enough detail to be reproducible. Be methodical in describing the
parts of the method that matter for reproducibility. But also be
concise. If the brand of a piece of equipment may be a factor in the results,
then state it. But, at the same time, don't provide irrelevant detail.

\subsection{Things to be particularly careful about in describing your methodology}

